A Formal Model to Facilitate Security Testing in Modern Automotive Systems

Ensuring a car's internal systems are free from security vulnerabilities is of utmost importance, especially due to the relationship between security and other properties, such as safety and reliability. We provide the starting point for a model-based framework designed to support the security testing of modern cars. We use Communicating Sequential Processes (CSP) to create architectural models of the vehicle bus systems, as well as an initial set of attacks against these systems. While this contribution represents initial steps, we are mindful of the ultimate objective of generating test code to exercise the security of vehicle bus systems. We present the way forward from the models created and consider their potential integration with commercial engineering tools

==> abstracts/keywords.tex <==
Formal Threat Model; Automatic Security Test Case Generation; Automotive Bus Systems; Vehicular Architectures; Automotive Security

==> eptcsdata.tex <==
\providecommand{\firstpage}{95}
\providecommand{\publicationstatus}{R. Laleau, D. M\'ery, S. Nakajima, E. Troubitsyna (Eds): Joint Workshop on\\ Handling IMPlicit and EXplicit knowledge in formal system development\\ and  Formal \& Model-Driven Techniques for Developing Trustworthy Systems.\\
EPTCS 271, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.271.7}{10.4204/EPTCS.271.7}}
\pdfoutput=1

